Embodied Agents for Efficient Exploration and Smart Scene Description

The development of embodied agents that can communicate with humans in natural language has gained increasing interest over the last years, as it facilitates the diffusion of robotic platforms in human-populated environments. As a step towards this objective, in this work, we tackle a setting for visual navigation in which an autonomous agent needs to explore and map an unseen indoor environment while portraying interesting scenes with natural language descriptions. To this end, we propose and evaluate an approach that combines recent advances in visual robotic exploration and image captioning on images generated through agent-environment interaction. Our approach can generate smart scene descriptions that maximize semantic knowledge of the environment and avoid repetitions. Further, such descriptions offer user-understandable insights into the robot's representation of the environment by highlighting the prominent objects and the correlation between them as encountered during the exploration. To quantitatively assess the performance of the proposed approach, we also devise a specific score that takes into account both exploration and description skills. The experiments carried out on both photorealistic simulated environments and real-world ones demonstrate that our approach can effectively describe the robot's point of view during exploration, improving the human-friendly interpretability of its observations.

==> sections/02-related.tex <==
\section{Related Work}

\tit{Embodied Navigation and Exploration} \label{em_explore}
A step forward to such diffusion would come from the introduction of explainability characteristics to allow the end-users to interpret the behavior of the state-of-the-art architectures tackling robotics perception and decision-making, which are generally considered black boxes. A possible strategy proposed in literature~\cite{cascianelli2018full,cornia2019smart,bigazzi2020explore,tan2022embodied} entails equipping the robot with a module that produces natural-language descriptions of its observations.

\tit{Image Captioning}\label{img_cap}
Image captioning is a task at the intersection between vision and language whose goal is to generate a natural language description of a given image. To represent images, convolutional neural networks can be used to extract global features~\cite{karpathy2015deep,rennie2017self}, grids of features~\cite{xu2015show,lu2017knowing}, or features for image regions containing visual entities~\cite{anderson2018bottom,lu2018neural}. 
In most cases, attention mechanisms are applied to enhance the visual input representation. More recent approaches employ fully-attentive Transformer-like architectures~\cite{vaswani2017attention} as visual encoders, which can also be applied directly to image patches~\cite{liu2021cptr,cornia2021universal,barraco2022camel}.
The image representation is used to condition a language model that generates the caption. The language model can be implemented as a recurrent neural network~\cite{karpathy2015deep,rennie2017self,huang2019attention,landi2021working} 
or Transformer-based fully-attentive models~\cite{cornia2020meshed,zhang2021rstnet}. 

In this work, we develop a fully-attentive image captioning approach as our captioning module, as it is potentially suitable to be employed in a wide variety of real-world settings such as embodied exploration.


